Practical Foundations of History Independence

The way data structures organize data is often a function of the sequence of past operations. The organization of data is referred to as the data structure's state, and the sequence of past operations constitutes the data structure's history. A data structure state can therefore be used as an oracle to derive information about its history. As a result, for history-sensitive applications, such as privacy in e-voting, incremental signature schemes, and regulatory compliant data retention; it is imperative to conceal historical information contained within data structure states. Data structure history can be hidden by making data structures history independent. In this paper, we explore how to achieve history independence. We observe that current history independence notions are significantly limited in number and scope. There are two existing notions of history independence -- weak history independence (WHI) and strong history independence (SHI). WHI does not protect against insider adversaries and SHI mandates canonical representations, resulting in inefficiency. We postulate the need for a broad, encompassing notion of history independence, which can capture WHI, SHI, and a broad spectrum of new history independence notions. To this end, we introduce $\Delta$history independence ($\Delta$HI), a generic game-based framework that is malleable enough to accommodate existing and new history independence notions. As an essential step towards formalizing $\Delta$HI, we explore the concepts of abstract data types, data structures, machine models, memory representations and history independence. Finally, to bridge the gap between theory and practice, we outline a general recipe for building end-to-end, history independent systems and demonstrate the use of the recipe in designing two history independent file systems.

==> hidstable.tex <==
\begin{table}[t]
%
%\vspace{0.2cm}
%\begin{center}
%\small
\tbl{Summary of history independent data structures. $\alpha$ $\leftarrow$ load factor,
$N$ $\leftarrow$ number of keys, $B$ $\leftarrow$ block transfer size. Also, 
I : insert, L : lookup, D : delete, R : range, P : predecessor, C : compare.\label{hitheory:table:existingresearch}}{%
\begin{tabular}{|c|c|c|c|}
\hline
{\bf Data Structure} & {\bf Year} & {\bf Ops} & {\bf Runtime}\\
\hline
2-3 Tree \cite{23tree} & 1997 & I,L,D & $O(\log N)$\\
\hline
Hash Table \cite{naorantipersistence} & 2001 & I,L & $O(log (1/(1-\alpha)))$\\
\hline
Hash Table \cite{blellochhashing} & 2007 & I,L,D & $O(1/(1-\alpha)^{3})$\\
\hline
Ordered & 2007 & I,P,D & $O(\log \log N)$\\
Dictionary \cite{blellochhashing} & & & \\
\hline
Order & 2007 & I,C,D & $O(1)$\\
Maintenance \cite{blellochhashing} & & & \\
\hline
Hash Table \cite{naorcuckoo} & 2008 & I,L,D & I,D $\rightarrow$ $O(\log N)$\\
& & & S $\rightarrow$ $O(1)$\\
\hline
B-Treaps \cite{golovinbtreaps} & 2009 & I,D,R & $O(log_B N)$\\
\hline
B-SkipList \cite{golovinbskiplist} & 2010 & I,D,R & $O(log_B N)$\\
\hline
R-Trees \cite{rtrees} & 2012 & I,D,R & n/a\\
\hline
\end{tabular}}	
\vspace{-0.2cm}
%\normalsize                      
%\caption{Summary of history independent data structures.
%\caption[Summary of history independent data structures]{Summary of history independent data structures. $\alpha$ $\leftarrow$ load factor,
%$N$ $\leftarrow$ number of keys, $B$ $\leftarrow$ block transfer size. Also, 
%I : insert, L : lookup, D : delete, R : range, P : predecessor, C : compare.
%\label{hitheory:table:existingresearch}}
%\vspace{-0.7cm}
%\end{center}
\end{table}


==> hifs/algos.tex <==
\section{Procedure Sets}
\label{hifs:algos}

%\input{hifs/custsequential}
%\vspace{2cm}
%\input{hifs/custnonfilesystem}
%\input{hifs/custinode}
\input{hifs/write}




==> hifs/custexample.tex <==
\begin{algorithm}[t]
\caption[Customizable Procedures for SHI with Block Group Locality]{Customizable Procedures for Block Group Locality}
\label{hifs:algorithm:custexample}
\textbf{Procedure:} GDB \\
\textbf{Desc:} get the logical file bucket number from file offset.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE file offset $f_{o}$ : $f_{o} \in \mathbb{N}$
\RETURN $\big( \big\lfloor \big\lfloor \frac{f_{o}}{d_{s}}\big\rfloor / d_{b_{n}} \big\rfloor \big)$
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
\textbf{Procedure:} GET\_MOST\_PREFERRED\_BUCKET\\
%\textbf{Desc:} get the top most bucket on key's preference list.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ : $k$ = \{file path $f_{p}$, file offset $f_{o}$\}
\RETURN \textless $h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$, $h(f_{p})$ mod $\mathsf{G_{n}}$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
\textbf{Procedure:} GET\_NEXT\_BUCKET\\
%\textbf{Desc:} get the next bucket on key's preference list.\\ 
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ : \{$f_{p}, f_{o}$\}, bucket $i$, block group $r$ : $(i,r) \in \mathbb{N}$
\STATE $i \leftarrow (i + 1)$ mod $\mathsf{B_{n}}$
\IF{$i == (h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$)}
	\STATE $r \leftarrow (r + 1)$ mod $\mathsf{G_{n}}$, $i \leftarrow h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$
\ENDIF
\RETURN  \textless$i,r$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} BUCKET\_PREFERS\\
%\textbf{Desc:} find which of two keys the given bucket prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE bucket i, block group r : (i,r)  $\in$ $\mathbb{N}$, key a : \{$f_{p_{a}}, f_{o_{a}}$\}, key b : \{$f_{p_{b}}, f_{o_{b}}$\}
\RETURN $h(f_{p_{a}}||$GDB$(f_{o_{a}}))$ \textgreater $h(f_{p_{b}}||$GDB$(f_{o_{b}}))$
\end{algorithmic}
%----------------------------------------------------------------------
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} KEY\_PREFERS\\
%\textbf{Desc:} find which of two buckets the given key prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key k : \{$f_{p}, f_{o}$\}, bucket i, bucket j, block group r, block group s : (i,j,r,s) $\in$ $\mathbb{N}$
\IF{r \textless\textgreater s}
	\RETURN (($h(f_{p})$ mod $\mathsf{G_{n}}$) - r + $\mathsf{G_{n}}$) mod $\mathsf{G_{n}}$ $\textless$ (($h(f_{p})$ mod $\mathsf{G_{n}}$) - s + $\mathsf{G_{n}}$) mod $\mathsf{G_{n}}$
\ENDIF
\RETURN (($h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$) - i + $\mathsf{B_{n}}$) mod $\mathsf{B_{n}}$ $\textless$ (($h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$) - j + $\mathsf{B_{n}}$) mod $\mathsf{B_{n}}$
\end{algorithmic}
\end{algorithm}
%%\vspace{-0.8cm}
%----------------------------------------------------------------------


==> hifs/custinode.tex <==
\begin{algorithm}[H]
\caption{Inode Table Customizable Procedures}
\label{hifs:algorithm:custinode}
\textbf{Procedure:} GET\_MOST\_PREFERRED\_BUCKET\\
%\textbf{Desc:} get the top most bucket on key's preference list.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = file path $f_{p}$
\RETURN \textless $h(f_{p})$ mod $\mathsf{I_{n}}$, $h(f_{p})$ mod $\mathsf{G_{n}}$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
\textbf{Procedure:} GET\_NEXT\_BUCKET\\
%\textbf{Desc:} get the next bucket on key's preference list.\\ 
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = $f_{p}$, bucket $i$, block group $r$
\STATE $i \leftarrow (i + 1)$ mod $\mathsf{I_{n}}$
\IF{$i == (h(f_{p})$ mod $\mathsf{I_{n}})$}
	\STATE $r \leftarrow (r + 1)$ mod $\mathsf{G_{n}}$, $i \leftarrow h(f_{p})$ mod $\mathsf{I_{n}}$
\ENDIF
\RETURN  \textless$i,r$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} BUCKET\_PREFERS\\
%\textbf{Desc:} find which of two keys the given bucket prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE bucket $i$, block group $r$, key $a$ = $f_{p_{a}}$, key $b$ = $f_{p_{b}}$
\RETURN $h(f_{p_{a}})$ $>$ $h(f_{p_{b}})$
\end{algorithmic}
%----------------------------------------------------------------------
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} KEY\_PREFERS\\
%\textbf{Desc:} find which of two buckets the given key prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = $f_{p}$, bucket $i$, bucket $j$, block group $r$, block group $s$
\IF{$r \neq s$}
	\RETURN (($h(f_{p})$ mod $\mathsf{G_{n}}) - r + \mathsf{G_{n}})$ mod $\mathsf{G_{n}} < ((h(f_{p})$ mod $\mathsf{G_{n}}) - s + \mathsf{G_{n}})$ mod $\mathsf{G_{n}}$
\ENDIF
\RETURN $((h(f_{p})$ mod $\mathsf{I_{n}}) - i + \mathsf{I_{n}})$ mod $\mathsf{I_{n}} < ((h(f_{p})$ mod $\mathsf{I_{n}}) - j + \mathsf{I_{n}})$ mod $\mathsf{I_{n}}$
\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------


==> hifs/custnonfilesystem.tex <==
\begin{algorithm}[H]
\caption[Customizable Procedures for Case C (External parameters)]{Customizable Procedures for Case C (External parameters) from Section \ref{hifs:architecture:filestorage:custhi}}
\label{hifs:algorithm:custnonfilesystem}
%\textbf{Procedure:} GDB \\
%%\textbf{Desc:} get the disk bucket from file offset.\\
%\vspace{-0.5cm}
%\begin{algorithmic}[1]
%\REQUIRE file offset $f_{o}$ : $f_{o}$ $\in$ $\mathbb{N}$
%\RETURN $\big( \big\lfloor \big\lfloor \frac{f_{o}}{d_{s}}\big\rfloor / d_{b_{n}} \big\rfloor \big)$
%\end{algorithmic}
%%
%%\vspace{-0.2cm}
%------------------------------------------------------------------ \\
\textbf{Procedure:} GET\_MOST\_PREFERRED\_BUCKET\\
%\textbf{Desc:} get the top most bucket on key's preference list.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ : $k$ = \{file path $f_{p}$, file offset $f_{o}$, user $u$\}
\RETURN \textless $h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}$, $h(u)$ mod $\mathsf{G_{n}}$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%\textbf{Procedure:} GET\_NEXT\_BUCKET\\
%%\textbf{Desc:} get the next bucket on key's preference list.\\ 
%\vspace{-0.5cm}
%\begin{algorithmic}
GET\_NEXT\_BUCKET and BUCKET\_PREFERS same
as in  procedure set \ref{hifs:algorithm:custexample}.\\
%%\REQUIRE key k : \{$f_{p}, f_{o}, u$\}, bucket i, block group r : (i,r) $\in$ $\mathbb{N}$
%\STATE same as in procedure set \ref{hifs:algorithm:custexample}.
%\end{algorithmic}
%%
%%\vspace{-0.2cm}
%------------------------------------------------------------------ \\
%%
%\textbf{Procedure:} BUCKET\_PREFERS\\
%%\textbf{Desc:} find which of two keys the given bucket prefers.\\
%\vspace{-0.5cm}
%\begin{algorithmic}
%\STATE same as in procedure set \ref{hifs:algorithm:custexample}.
%\end{algorithmic}
%----------------------------------------------------------------------
%
%\vspace{-0.1cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} KEY\_PREFERS\\
%\textbf{Desc:} find which of two buckets the given key prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ : \{$f_{p}, f_{o}, u$\}, bucket $i$, bucket $j$, block group $r$, block group $s$ : $(i,j,r,s) \in \mathbb{N}$
\IF{$r \neq s$}
	\RETURN $((h(u)$ mod $\mathsf{G_{n}}) - r + \mathsf{G_{n}})$ mod $\mathsf{G_{n}} < ((h(u) mod \mathsf{G_{n}}) - s + \mathsf{G_{n}})$ mod $\mathsf{G_{n}}$
\ENDIF
\RETURN $((h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}) - i + \mathsf{B_{n}})$ mod $\mathsf{B_{n}} < ((h(f_{p}||$GDB$(f_{o}))$ mod $\mathsf{B_{n}}) - j + \mathsf{B_{n}})$ mod $\mathsf{B_{n}}$
\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------


==> hifs/custsequential.tex <==
\begin{algorithm}[H]
\caption[Customizable Procedures for Case B (Complete Sequential)]{Customizable Procedures for Case B (Complete Sequential) from Section \ref{hifs:architecture:filestorage:custhi}}
\label{hifs:algorithm:custsequential}
%\textbf{Procedure:} GDB \\
%\textbf{Desc:} get the disk bucket from file offset.\\
%%\vspace{-0.5cm}
%\begin{algorithmic}[1]
%\REQUIRE file offset $f_{o}$ : $f_{o}$ $\in$ $\mathbb{N}$
%\RETURN $\big( \big\lfloor \big\lfloor \frac{f_{o}}{d_{s}}\big\rfloor / d_{b_{n}} \big\rfloor \big)$
%\end{algorithmic}
%%
%%\vspace{-0.2cm}
%------------------------------------------------------------------ \\
\textbf{Procedure:} GET\_MOST\_PREFERRED\_BUCKET\\
\textbf{Desc:} get the top most bucket on key's preference list.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = \{file path $f_{p}$, file offset $f_{o}$\}
\RETURN \textless$0, h(f_{p})$ mod $\mathsf{G_{n}}$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
\textbf{Procedure:} GET\_NEXT\_BUCKET\\
\textbf{Desc:} get the next bucket on key's preference list.\\ 
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = \{$f_{p}, f_{o}$\}, bucket $i$, block group $r$
\STATE $i \leftarrow (i + 1)$ mod $\mathsf{B_{n}}$
\IF{$i == 0$}
	\RETURN \textless$0, (r + 1)$ mod $\mathsf{G_{n}}$\textgreater
\ENDIF
\RETURN  \textless$i,r$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} BUCKET\_PREFERS\\
\textbf{Desc:} find which of two keys the given bucket prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE bucket $i$, block group $r$, key $a$ = \{$f_{p_{a}}, f_{o_{a}}$\}, key $b$ = \{$f_{p_{b}}, f_{o_{b}}$\}
\IF {$f_{p_{a}} == f_{p_{b}}$}
	\RETURN GDB$(f_{o_{a}}) < $GDB$(f_{o_{b}})$
\ENDIF
\RETURN $h(f_{p_{a}})$ \textgreater $h(f_{p_{b}})$
\end{algorithmic}
%----------------------------------------------------------------------
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} KEY\_PREFERS\\
\textbf{Desc:} find which of two buckets the given key prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ = \{$f_{p}, f_{o}$\}, bucket $i$, bucket $j$, block group $r$, block group $s$
\IF{$r \neq s$}
	\RETURN $((h(f_{p})$ mod $\mathsf{G_{n}}) - r + \mathsf{G_{n}})$ mod $\mathsf{G_{n}} < ((h(f_{p})$ mod $\mathsf{G_{n}}) - s + \mathsf{G_{n}})$ mod $\mathsf{G_{n}}$
\ENDIF
\RETURN $i < j$ 
\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------


==> hifs/dafsparameters.tex <==
\small
\begin{tabular}{|c|c|}
%\begin{|p{1.8cm}|c|p{5cm}|p{7cm}|c|}
\hline
{\bf Parameter}	& {\bf Value}\\
\hline
File system size & 10 GB\\
\hline
Mean database size & 1 GB\\
\hline
No. of databases & $\mathit{L} \cdot 10$\\
\hline
Disk block size ($\mathsf{d_{s}}$) & 4 KB\\
\hline
No. of block groups ($\mathsf{G_{n}}$) & 4\\
\hline
Disk blocks per bucket ($\mathsf{d_{b_{n}}}$) & 512\\
\hline
Inode size & 281 bytes\\
\hline
\end{tabular}
\normalsize


==> hifs/demo.tex <==
\section{HIFS Visualizer (Demo)}
\label{hifs:demo}

%
\label{hifs:demo}
\begin{figure}[t]
\begin{center}
\vspace{-0.2cm}
%\includegraphics[scale=0.65]{hifs/figures/demo.eps}
\includegraphics[width=17cm,height=15cm]{hifs/figures/demo.eps}
\vspace{-0.7cm}
\caption{HIFS Visualizer.}
\label{hifs:figure:demo}
\vspace{-0.8cm}
\end{center}
\end{figure}
%
The HIFSVisualizer (Figure \ref{hifs:figure:demo}) aids in the demonstration and understanding of history
independent storage in HIFS. For a given history independent layout and
number of files it visualizes the entire disc image. Users can also
select different history independent layouts and see how changes in
the file creation sequence results in the same canonical 
(i.e., history independent) layouts in HIFS.


==> hifs/discussion.tex <==
\section{Discussion}
\label{hifs:discussion}
%
%\subsection{Secure Deletion}
%\label{hifs:discussion:securedeletion}
%\subsubsection{Data Shredding}
%%
%When an element is deleted from a history independent implementation it is imperative
%that proper data shredding is employed, that is, the data at the location is
%made irrecoverable (e.g., by overwriting \cite{sok}).  Any residual data
%artifacts can compromise the history of operations.  Hence, \emph{HIFS} does
%not mark hash table entries as deleted but immediately performs an overwrite
%on each delete operation.  This applies to all history independent disk
%structures (inode table, disk bucket maps) and to the file data
%blocks.

%\subsection{Temporal Meta-data}
%\label{hifs:discussion:temporal}
%\subsubsection{Temporal Meta-data}
%%
%File systems typically maintain temporal meta-data such as modification times
%(for files and directories) which are then made available
%to applications.
%% via interfaces.
%For certain composite applications it may
%be desired that the history of operations across files is also private. 
%\emph{HIFS} can optionally be configured to provide such functionality,
%which it does by (a) not maintaining any temporal meta-data for files, and
%(b) using history independent directories.
%
%%A directory is a special file whose contents are the list of files present
%%in that directory.
%A directory file consists of a set of directory
%entries, one entry for each file in that directory.  If cross-file history
%independence is desired then \emph{HIFS} maintains the contents of each
%directory file in a history independent manner.  For this, no additional
%data structures are employed, instead the directory entries are always
%stored sorted.  Since a simple sorted list is history independent
%\cite{naorantipersistence} the sorting of directory contents suffices.
%
%\subsection{Limitations}
%\label{hifs:architecture:limitations}
%\subsection{System failure and Recovery}
%%
%File system operations access multiple
%disk data structures which cannot all be updated simultaneously.
%Hence, in case of an inopportune system failure, the history independence
%related to certain records can be violated. For example, consider a file
%delete operation that accesses file system data structures in the
%following sequence --
%(a) deletes file inode entry from the inode table,
%(b) deletes an entry from the disk buckets map, and
%(c) deletes file contents from the corresponding disk bucket.
%Now, suppose that a system failure occurs after step (b) and an adversary
%gains access to the disk layout at this exact moment.
%By examining the disk buckets map and the data blocks on disk, the adversary
%%can deduce that the last operation was a delete. 
%% Thus information that is not
%% otherwise accessible via file system interface is revealed.
%%However, once the system recovers from failure history independence is restored.
%
%Existing recovery mechanisms such as journaling can be utilized to
%efficiently restore system consistency after a failure.
%However, we note that this breaks history independence since the
%adversary can potentially gain information about the recent operations. 
%In case of journaling data can reside on disk without the associated updated meta-data
%(or vice versa). Hence data residing on disk with stale or missing meta-data is
%likely to be identified as recently written.
%%log based
%%recovery will reveal at least the last file system operation. 
%Designing efficient recovery mechanisms that completely preserve history independence
%remains an open problem.
%
\subsection{In-Memory History Independence}
% 
\emph{HIFS} protects history independence only for data residing on disk.
It does not target in-memory structures such as the file system cache.

Although the need for a history independent memory allocator for in-memory
data structures has been voiced \cite{golovinthesis}, we posit that
extension of history independence to data in memory requires further careful
examination. Simply replacing in-memory caches with history independent
versions will not suffice.
Firstly, an in-memory system cache cannot treat each disk block
independently, but instead needs to maintain inter-block associations.
For example, it must avoid scenarios such as the disk buckets map is
written to disk but the modified file data blocks still reside
in the cache for a significant time interval after. This can potentially
reveal to an adversary details about the last file operation performed.
Further, the relationships between in-memory data and its disk copies in a
history independent context need to be investigated. This includes not just
file system cache and data structures but also other system components such
as the operating system kernel and low level system caches.

%\noindent
%{\bf Caching.~}
%Since system memory is not targeted in this work the file system cache
%is yet not history independent. 

% In subsequent works we will extend history independence to memory and
% other system components.

%\subsection{Storage Media}
%%
%%HIFS is designed for storage devices (disks) that expose block placement to
%%upper layers.
%HIFS does not provide history independence if deployed (as
%is) on top of devices that manage their own internal block placement, such
%as SSDs, due to the wear-leveling mechanisms.
%The flash firmware's relocation of data blocks (wear leveling) is aimed to
%increase the life span of the drive.
%This essential functionality of the flash controller directly contradicts
%with history independence, since history independence requires fixed layouts.
%As of today we do not know how to reconcile both. Hence in HIFS we only
%focus on hard disk devices.

%Hence we cannot expect this functionality to
%be removed. Even if a lower-layer interface is exposed
%movement of blocks will have to be carried out to avoid hot spots.

%, since that would defeat any HIFS provided assurances.

%- list all features from Ext2 that are not yet supported by \emph{HIFS}
%e.g. hard / soft links

%further customization : preferences. disk bucket size 
%block group size - what should the above values be for
%different applications e.g. web server, large files,
%infrequent file growth sequential etc

%future work
%- in memory hi
%- new hids or use other than ht


==> hifs/hifs.tex <==
\chapter{History Independent File System}
\label{chapter:hifs}

%Although our primary motivation to seek history independence
%was secure deletion, we note 

\input{hifs/intro}
\input{hifs/model}
\input{hifs/concepts}
%\input{hifs/motivation}	%do not include
\input{hifs/architecture}
\input{hifs/discussion}
\input{hifs/experiments}
\input{hifs/related}
\input{hifs/demo}
\input{hifs/conclusion}
\input{hifs/algos}



==> hifs/hifsproof.tex <==
\subsection{Proofs of History Independence}
\label{hifs:architecture:proofs}
% 
Let $K$ denote the set of keys and $\beta$ denote the buckets within the
hash table.  Also, let $k.pref(b)$ denote bucket $b$'s position on key $k$'s
preference list ($k \in K$ and $b \in \beta$) where, lower value of $k.pref$
indicates higher preference.  Then, we have the following definition

\begin{definition}
{\em Un-ambiguous Preferences} \\
A set of preferences from $K \rightarrow \beta$ and $\beta \rightarrow K$
are {\em un-ambiguous} if\\
(a) $\forall k \in K$, $\nexists$ $(b_{i},b_{j}) \in \beta$, $i \neq j$ s.t.
$k.pref(b_{i}) = k.pref(b_{j})$\\
and\\
(b) $\forall b \in \beta$, $\nexists$ $(k_{i},k_{j}) \in K$, $i \neq j$ s.t.
$b.pref(k_{i}) = b.pref(k_{j})$.

\end{definition}

\begin{thm}
\label{hifs:theorem:hiexample}
%
The customizable procedures listed in Procedure Set
\ref{hifs:algorithm:custexample} result in a history independent hash table
with unique representation.
%
\end{thm}

\begin{proof}
%
The Gale-Shapley Stable Marriage algorithm \cite{galeshapley} has shown that
if (a) men propose in decreasing order of their preference, and (b) all
preferences are un-ambiguous, then the resulting stable matching is unique.
\cite{blellochhashing} then showed that the hash table discussed in Section
\ref{hifs:architecture:hiht} satisfies both (a) and (b). They then proved
that as a result the distribution of keys in the hash table is canonical and
thus history independent.
Thus, distributions from any set of customizable procedures
are history independent 
% using proofs as in \cite{blellochhashing} 
if they exhibit the above two properties.

We now detail this for the customizable procedures in Procedure Set
\ref{hifs:algorithm:custexample} applicable to case A (Block Group Locality)
from Section \ref{hifs:architecture:filestorage:hi}.

\subsubsection{(a) Proposal Order}
%
Each time a new key is inserted in to the hash table, the first attempt is
to place the key in its most preferred bucket i.e.  bucket $b$ where
$k.pref(b)$ is minimum (see procedure INSERT in set
\ref{hifs:algorithm:hiht} which foremost calls GET\_MOST\_PREFERRED\_BUCKET
in set \ref{hifs:algorithm:custexample}).  Each new bucket in the probe
sequence is selected by the procedure GET\_NEXT\_BUCKET which given a bucket
$b_{i}$ finds the bucket $b_{j}$ such that $\nexists$ $b_{l}$ where
$k.pref(b_{i}) < k.pref(b_{l}) < k.pref(b_{j})$.  In other words $b_{j}$ is
always the next preferred bucket on key $k$'s preference list.  Thus
analogous to men in the stable marriage algorithm the matching of keys to
buckets is attempted in decreasing order of key preferences.

\subsubsection{(b) Un-ambiguous preferences}
% 
A bucket's preference between two keys is resolved in BUCKET\_ PREFERS using
the condition
$h(f_{p_{a}}||$GDB$(f_{o_{a}}))$\textgreater$h(f_{p_{b}}||$GDB$(f_{o_{b}}))$. 
Hence, if the two values compared above are always distinct then the
comparison is un-ambiguous.  We note that for any given set of files
$\mathit{F}$ the combination of the file path and the logical file bucket
number is unique, that is, $\forall f \in F$,
\textless$f_{p},$GDB$(f_{o})$\textgreater is unique.  Hence, the hash value
$h(f_{p}||$GDB$(f_{o}))$ is unique.  The proof then reduces to collision
resistance of the hash function (e.g., SHA \cite{sha1}).

Similarly, a key's preference amongst two buckets is resolved by the
procedure KEY\_PREFERS.  Here, firstly if the two buckets belong to separate
block groups (line 1) then the key simply prefers the bucket in the block
group with the lower index (line 2).  Hence, this condition is un-ambiguous. 
If the two buckets are in the same block group, then the key prefers the
bucket closer to its most preferred bucket in that block group (line 3).
Again, since the comparison is based on the hash of the unique combination
\textless$f_{p},$GDB$(f_{o})$\textgreater the proof reduces to collision
resistance of the hash function.
%
\end{proof}

Similar proofs exist for the customizable procedures of cases B and C from
Section \ref{hifs:architecture:filestorage:custhi}, and for the inode table.


==> hifs/hihtalgorithm.tex <==
%\vspace{0.4cm}
\begin{algorithm}[t]
\caption{History Independent Hash Table}
\label{hifs:algorithm:hiht}
\textbf{Procedure: } INSERT\\
\textbf{Desc:} insert the given key in to the hash table.\\
\vspace{-0.5cm} 
\begin{algorithmic}[1]
\REQUIRE Tables $H^{0-m}[n]$, key $k$
\STATE	\textless$i,r$\textgreater $\leftarrow$ GET\_MOST\_PREFERRED\_BUCKET($k$)
\STATE $c \leftarrow 0$
\WHILE{$c < (n * (m + 1))$}
	\IF{$H^{r}[i]$ is null}
		\STATE		$H^{r}[i] \leftarrow k$
		\RETURN		\textless$i,r$\textgreater
	\ENDIF
	\IF{BUCKET\_PREFERS($i, r, k, H^{r}[i]$)}
		\STATE	SWAP($k, H^{r}[i]$)
	\ENDIF
	\STATE	\textless$i,r$\textgreater $\leftarrow$ GET\_NEXT\_BUCKET($k, i, r$)
	\STATE $c \leftarrow c + 1$
\ENDWHILE
\RETURN \textless$null,null$\textgreater	\quad \COMMENT{tables are full}
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure: } SEARCH\\
\textbf{Desc:} search for the given key in the hash table.\\
\vspace{-0.5cm} 
\begin{algorithmic}[1]
\REQUIRE Tables $H^{0-m}[n]$, key $k$
\STATE	\textless$i,r$\textgreater $\leftarrow$ GET\_MOST\_PREFERRED\_BUCKET($k$)
\STATE $c \leftarrow 0$
\WHILE{$c < (n * (m + 1))$ AND $H^{r}[i]$ is not null}
	\IF{k == $H^{r}[i]$}
		\RETURN \textless$i,r$\textgreater	\quad \COMMENT{key found at $H^{r}[i]$}
	\ENDIF
	\STATE	\textless$i,r$\textgreater $\leftarrow$ GET\_NEXT\_BUCKET($k, i, r$)
	\STATE $c \leftarrow c + 1$
\ENDWHILE
\RETURN \textless$null,null$\textgreater	\quad \COMMENT{key not found}
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure: } DELETE\\
\textbf{Desc:} delete the given key from the hash table.\\
\vspace{-0.5cm} 
\begin{algorithmic}[1]
\REQUIRE Tables $H^{0-m}[n]$, key $k$
\STATE	\textless$i,r$\textgreater $\leftarrow$ SEARCH($k$)
\WHILE{$i$ is not null AND $H^{r}[i]$ is not null}
	\STATE \textless$j,s$\textgreater $\leftarrow$ GET\_NEXT\_BUCKET($k, i, r$)
	\IF{$H^{s}[j]$ is not null AND KEY\_PREFERS( $H^{s}[j], i, j, r, s$)}
		\STATE $H^{r}[i] \leftarrow H^{s}[j]$
		\STATE $k \leftarrow H^{s}[j]$
		\STATE $i \leftarrow j, r \leftarrow s$
	\ENDIF
\ENDWHILE
\end{algorithmic}
\end{algorithm}
%\vspace{0.4cm}
%-------------------------------------------------------------------------------


==> hifs/hihtalgorithmcust.tex <==
%\vspace{0.2cm}
\begin{algorithm}[t]
\caption{Customizable Procedures \cite{blellochhashing}}
\label{hifs:algorithm:hihtcust}
\textbf{Procedure:} GET\_MOST\_PREFERRED\_BUCKET\\
\textbf{Desc:} get the top most bucket on key's preference list.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$ : $k \in \mathbb{N}$
\RETURN \textless$k$ mod $n, 0$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
\textbf{Procedure:} GET\_NEXT\_BUCKET\\
\textbf{Desc:} get the next bucket on key's preference list.\\ 
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$, bucket $i$, table $r$ : $(k,i,r) \in \mathbb{N}$
\STATE $i \leftarrow (i + 1)$ mod $n$
\IF{$i == (k$ mod $n)$}
	\STATE $r \leftarrow r + 1$
	\STATE $i \leftarrow k$ mod $n$
\ENDIF
\RETURN  \textless$i,r$\textgreater
\end{algorithmic}
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} BUCKET\_PREFERS\\
\textbf{Desc:} find which of two keys the given bucket prefers.\\
\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE bucket $i$, table $r$, key $a$, key $b$ : $(i,r,a,b) \in \mathbb{N}$
\RETURN $a > b$
\end{algorithmic}
%----------------------------------------------------------------------
%
%\vspace{-0.2cm}
--------------------------------------------------------------------------------------------------------------\\
%
\textbf{Procedure:} KEY\_PREFERS\\
\textbf{Desc:} find which of two buckets the given key prefers.\\
%\vspace{-0.5cm}
\begin{algorithmic}[1]
\REQUIRE key $k$, bucket $i$, bucket $j$, table $r$, table $s$ : $(k,i,j,r,s) \in \mathbb{N}$
\IF{$r \neq s$}
	\RETURN $r < s$
\ENDIF
\RETURN $((k$ mod $n) - i + n)$ mod $n < ((k$ mod $n) - j + n)$ mod $n$
\end{algorithmic}
\end{algorithm}
%----------------------------------------------------------------------


==> hifs/motivation.tex <==
\section{History Independence}
\label{hifs:motivation}

%
\begin{figure}[t]
\begin{center}
\vspace{2cm}
\includegraphics[scale=0.4]{hifs/figures/btreenohi.eps}
\vspace{-6.9cm}
\caption{B-Tree, a non history independent data structure.\label{fig:hifs:btreenohi}}
\vspace{-0.8cm}
\end{center}
\end{figure}
%
\subsection{File Systems}
\label{hifs:motivation:filesystems}
%
%A File System \cite{filesystem} provides storage of and access to a set of files.
%This functionality is made available to users and applications via specific interfaces 
%(open, create, read, write etc). In addition, the file system also maintains meta-data for
%its files (for access control, free space management etc).

%File systems organize file(s) data on disk. For existing file systems, the disk
Existing file systems do not preserve history independence because
the disk layouts they produce are not just a function of file contents
but also depend on the sequence of file operations. The exact same set
of files can be organized differently on disk depending on the
sequence of operations that created the set. 
%Existing file systems are therefore history dependent.
As a result, a simple examination of the disk layouts can reveal sensitive
information about past operations.
%, such as evidence of a file delete operation performed in the past.
Moreover, the data structures used to maintain file system meta-data also
contain information about past operations, both in their layouts, and
in their contents (e.g., list of allocated blocks).
Therefore, when disk layouts are combined with file system meta-data
and knowledge of data structures that are stored within files,
significantly more information can be derived, even full recovery of
deleted data.
% in the past.
Such leakage can violate secure deletion requirements and compromise
privacy in applications such as e-voting. 

At first it may appear that a simple replacement of all file system
data structures (file meta-data, free block list etc) 
with their history independent versions would suffice to resolve the
issue and preserve privacy. However, this is not the case, for the
privacy leaks are not due to the data itself but due to the
organization of data on disk.
File system encryption too cannot solve the problem since the concern
here is not data confidentiality. The relevant adversary is in fact an
insider that requires and is rightfully granted full access to the data
in the future (including disk encryption keys etc) and thus can easily
bypass any protections encryption may offer.
The solution then is to make file systems completely history independent.
The disk layouts of a history independent file system (defined in Section
\ref{hifs:motivation:filesystems:definition}) are only a function of data
and not of the sequence of past operations.
%A history independent file system will produce the exact same disk
%layouts for a given set of files irrespective of the operations that
%create the set.

%The data structures that are used to maintain file system meta-data are
%contain information about past operations in their layouts.

%In this section we would like to drive home the point that simply deploying
%history independent data structures at the application layer does not
%suffice to ensure secure deletion unless the underlying file system is also
%history independent.

%
\begin{figure}[t]
\begin{center}
\vspace{2.3cm}
\includegraphics[scale=0.55]{hifs/figures/btreenohidisklayout1.eps}
\vspace{-5.9cm}
\caption[B-Treaps and file system layouts, example one]{B-Treaps and file system layouts. $I_{R}(t)$ and $D_{R}(t)$ denote insertion and deletion respectively of element $t$ in relation $R$.
\label{fig:hifs:btreenohidisklayouts1}}
\vspace{-0.8cm}
\end{center}
\end{figure}
%
%
\begin{figure}[t]
\begin{center}
\vspace{3cm}
\includegraphics[scale=0.45]{hifs/figures/btreenohidisklayout2.eps}
\vspace{-6cm}
\caption[B-Treaps and file system layouts, example two]{B-Treaps and file system layouts. $I_{R}(t)$ and $D_{R}(t)$ denote insertion and deletion respectively of element $t$ in relation $R$.
\label{fig:hifs:btreenohidisklayouts2}}
\vspace{-0.8cm}
\end{center}
\end{figure}
%
%\begin{figure*}[t]
%\begin{center}
%\vspace{1.2cm}
%\hspace{-0.5cm}
%\includegraphics[scale=0.55]{hifs/figures/btreenohidisklayout1.eps}
%%\vspace{-3cm}
%\includegraphics[scale=0.55]{hifs/figures/btreenohidisklayout2.eps}
%%\hspace{-1cm}
%\vspace{-3.7cm}
%\caption{B-Treaps and file system layouts. $I_{R}(t)$ and $D_{R}(t)$ denote insertion and deletion respectively of element $t$ in relation $R%$.
%\label{fig:hifs:btreenohidisklayouts}}
%\vspace{-0.8cm}
%\end{center}
%\end{figure*}
%

%\noindent
%{\bf Need for History Independent Data Structures.~}
%--------------------------------------------------------------------------------
\subsubsection{Example Illustration}
To illustrate the need for history independence in file systems we consider an
admissions management application at a hospital
that records patients' data as new patients are admitted. The application
API permits the hospital staff to add new patient records, lookup existing
records and delete patient records on discharge.
We will use this example for illustration but note that in essence, most
existing applications of history independent data structures
%\cite{naorcuckoo,naorantipersistence,blellochhashing,molnarprom,moranwriteonce,ficklebase}
cannot be securely realized in practice without an underlying file system
providing history independent persistence.

%\subsection{Data Structures}
The patient application will typically utilize a database to manage its
data. Now, a database in turn stores and manipulates data by utilizing
efficient data structures of which B-Trees \cite{btree} are the most common
example. However, the use of B-Trees causes several privacy concerns.
This is because the storage layout of B-Trees (or of variations such as B$^{+}$-Trees)
often depends on the order in which operations are performed on them due to
their deterministic insertions and deletions. For example, consider
the the illustration in Figure \ref{fig:hifs:btreenohi}, which shows
two B-Trees that store the exact same elements. Yet the layouts of the two
B-Trees differ due to different insertion orders.
Hence, simply by examining the tree layout (Figure
\ref{fig:hifs:btreenohi}(a)) one can ascertain with a probability of 75\%
that \emph{Chad} was admitted before \emph{John}. This is due to the fact
that out of the total 4! ways of insertion for the four elements
\emph{Adam, Chad, John and Katy}, \emph{Chad} is the root in only
twelve, and inserted before \emph{John} in nine of those twelve sequences.

% Note that the application API over the B-Tree permits only
% insertions, deletions and lookups, and hence reveals nothing
% about the order of insertions in the tree. Hence, the information
% gained
% %by the adversary
% from the tree layout is external to the exposed API.
% %
% %For B-Trees in particular the risk of disclosure regarding past
% %operations does decrease as the fan-out increases and fan-outs in
% %typical usages are usually large.
% %Hence, although such deductions are difficult in practice,
% %hey are nonetheless possible and in certain specific cases trivial \cite{kiesebergtreesfa}. 

%\noindent
%{\bf Need for History Independent File System.~}
%\subsection{File System}
%
The above limitation of B-Trees can be prevented by deploying
corresponding history independent versions, such as B-Treaps \cite{golovinbtreaps}.
%\footnote{History Independence is more formally defined in \cite{blellochhashing,hartlinecharacterizinghi}.}.
The treaps will yield the same layout irrespective of the insertion order.
However, such a simple replacement of application data structures with their
history independent versions does not suffice unless the underlying
persistent mechanisms (e.g., file system) are also history independent.
To clarify, suppose that the B-Trees from above are replaced by the history
independent B-Treaps \cite{golovinbtreaps}.  Also, suppose that the
application has two relations, one for admissions to the General ward and
another for admissions to the Special ward, and that both relations are
persisted using a simple file system that allocates the first available free
block on request (and is hence not history independent). For simplicity,
assume that the B-Treap node size is equal to the file system block size.

Now, consider the sequence of operations, the resultant B-Treaps, and the
space allocation by the underlying file system as shown in Figure
\ref{fig:hifs:btreenohidisklayouts1}.
At the end of operation 7, the disk layout (Figure
\ref{fig:hifs:btreenohidisklayouts1}) reveals the following.  (i) The fact
that a delete operation was performed.  The gaps left by the file system
allocation form evidence for a delete.  (ii) That the deleted node belonged
to the General relation.  Since otherwise there would be no gaps in the file
system.  (iii) The first patient was not admitted to the Special ward, since
the root node of Special relation is not the first block on storage.
Note that neither the layout of the B-Treaps nor the application API reveal
any of (i) - (iii). The leaks are solely due to file system allocation.

Figure \ref{fig:hifs:btreenohidisklayouts2} shows an alternate sequence of
operations that yield the exact same trees as in Figure
\ref{fig:hifs:btreenohidisklayouts1} yet with significantly different disk
layouts, showing that the disk layouts produced by the file system allocation
heavily depend on file system operation sequencing. Hence, underlying storage mechanisms
can defeat the history independence of higher level data structures.

While we used a simple file system scenario for illustration, we note that 
%all practical
existing file systems (e.g., Ext2/Ext3 \cite{ext2}) suffer
from the same problems, since, for efficiency, and to preserve locality, 
they too allocate new blocks based on existing state, resulting in heavily
history dependent layouts. 
A history independent file system on the other hand would reveal none of (i) to
(iii) above since it would carry no evidence of a delete, such as gaps in block
allocation. Similarly, its allocation policy would not be dependent on the
order of file operations, resulting in the exact same disk layouts for the
operation sequences of both Figures \ref{fig:hifs:btreenohidisklayouts1}
and \ref{fig:hifs:btreenohidisklayouts2}.
%--------------------------------------------------------------------------------
\subsubsection{History Independent File System}
\label{hifs:motivation:filesystems:definition}
%
Let $\Psi^{\Gamma}_{\mathit{F}}$ denote the distribution
(layout) over secondary storage of the state $\mathit{F}$, of a file system
$\Gamma$.
%, $\mathit{|F|} \ge 0$. 
$\mathit{F}$ represents all file contents plus meta-data for individual
files and for the overall file system. Also, let $S^{\Gamma}_{\mathit{F}
\rightarrow \mathit{F'}}$ denote a set of operations
performed by file system $\Gamma$ transforming its state from $\mathit{F}$
into $\mathit{F'}$. We can then define the following.
%
\begin{definition}
\label{hifs:def:hifs}
{\em History Independent File System (HIFS)} \\
$\Gamma$ is a history independent file system if any two sequence
of operations $X^{\Gamma}_{\mathit{F} \rightarrow \mathit{F'}}$ and
$\mathit{Y}^{\Gamma}_{\mathit{F} \rightarrow \mathit{F'}}$ result in an
identical distribution $\Psi^{\Gamma}_{\mathit{F'}}$.
\end{definition}
% 
Formulated differently, for two sequences of operations $X^{\Gamma}_{\mathit{F}
\rightarrow \mathit{F'}}$ and $\mathit{Y}^{\Gamma}_{\mathit{F} \rightarrow
\mathit{F'}}$, an adversary having access to both the start state $\mathit{F}$
and the end state $\mathit{F'}$, should not be able to deduce which of $X$ or
$Y$ was executed to transform the state from $\mathit{F}$ into $\mathit{F'}$. 
%\footnote{Arbitrary more or less formal and convoluted definitions (when and
%how does the adversary have access to the states etc.) can be
%introduced here to capture different sub-scenarios, but we chose not to do
%so now since this is a systems paper and this definition captures a strong
%adversary and a relevant deployment.}
%Reconsidering the examples from Section \ref{hifs:motivation}, a history independent
%file system as per this definition, will generate the same layout on disk for
%the sequence of operations in Figures \ref{fig:hifs:btreenohidisklayouts}(a) and
%\ref{fig:hifs:btreenohidisklayouts}(b).
%
It can be easily seen that satisfying this definition immediately implies
that, the data at a particular offset of any file $f$ in $\mathit{F}$, is
always stored at the same device-specific location, irrespective of the
sequence of operations that result in $\mathit{F}$. That is, the representation of
the state $\mathit{F}$ over the storage medium is canonical.
%More on this later. 

% In summary, to ensure complete storage privacy, history independent data structures
% need to be persisted only using history independent File systems.
%--------------------------------------------------------------------------------
%\noindent
%{\bf General Case.~}
\subsection{System-Wide History Independence}
%
%So far, we have presented the specific case wherein the information
%protected by the application layer is compromised due to the properties of
%the lower-level file system layer.  Also, HIFS only targets these two layers.
%However, while out of scope, it may we worth to briefly generalize. 
Although detailed discussion is out of scope, we briefly generalize
history independence for an entire system.

Consider a typical system composed of multiple layers, ranging from
software applications to hardware (Figure \ref{fig:hifs:hifsneed}).
%These examples can be easily extended to any two system layers, 
%thereby further bolstering the need for system-wide history
%independence. 
Let these layers be denoted by $\mathit{L^{0}}$, $\mathit{L^{1}}$, $\mathit{L^{2}}$ etc,
where $\mathit{L^{0}}$ is the bottom layer, $\mathit{L^{1}}$ the next higher 
layer and so on. Also, let $S^{\mathit{L^{i}}}_{\mathit{A} \rightarrow \mathit{B}}$
denote the set of operations that transform $\mathit{L^{i}}$ from state $\mathit{A}$
to $\mathit{B}$. Further suppose that, for each state $\mathit{A}$ of $\mathit{L^{i}}$,
there exists a state $\mathit{A'}$ of $\mathit{L^{i-1}}$ with the
requirement that when $\mathit{L^{i}}$ is in state $\mathit{A}$, $\mathit{L^{i-1}}$ must be in state
$\mathit{A'}$ -- we denote this relationship between $\mathit{A}$ and $\mathit{A'}$
as $\mathit{L^{i}_{A}} \rightarrow \mathit{L^{i-1}_{A'}}$. Then we can
define the following.
%
\begin{definition}
\label{hifs:def:hisys}
{\em History Independent System} \\
A system is history independent if (i) each system layer $\mathit{L^{i}}$ is history independent, $i \ge 0$, and
(ii) any sequence of operations
$X^{\mathit{L^{i}}}_{\mathit{A} \rightarrow \mathit{B}}$ causes $\mathit{L^{i-1}}$
to change from state $\mathit{A'}$ to $\mathit{B'}$, where 
$\mathit{L^{i}_{A}} \rightarrow \mathit{L^{i-1}_{A'}}$,
$\mathit{L^{i}_{B}} \rightarrow \mathit{L^{i-1}_{B'}}$ and
$i > 0$.
\end{definition}

%
%
%\begin{figure}[t]
%\begin{center}
%\vspace{2cm}
%\includegraphics[width=8.5cm,height=7.5cm]{hifs/figures/btreenohidisklayout2.eps}
%\vspace{-6cm}
%\caption{B-Tree and file system layouts, insert-only operations.\label{fig:hifs:btreenohidisklayout12}}
%\vspace{-0.7cm}
%\end{center}
%\end{figure}
%
%which depicts
%the disk allocation by a simple file system that allocates the first available free block on a
%write and is thus not history independent. The operation sequences in Figures
%\ref{fig:hifs:nohifs}(a) and \ref{fig:hifs:nohifs}(b) both create the same files with the
%same content on disk. However, the layout of file contents on disk differs due to file system policy.
%Hence, an adversary with access to the disk can (by observing the disk layout) 
%determine the actual write sequence.
%Similarly, the sequences in Figures \ref{fig:hifs:nohifs}(c) and \ref{fig:hifs:nohifs}(d)
%are easily distinguishable by inspecting the disk allocation. Moreover, the resultant disk
%layout in Figure \ref{fig:hifs:nohifs}(c) by itself reveals the fact that a file delete
%operation was performed although no file system interface lists this information.


==> hifs/parameters.tex <==
%\begin{table}[t]
%\tbl{Experimental parameters. L $\leftarrow$ File System Load factor.
%\label{hifs:table:expparameters}}{%
\small
\begin{tabular}{|c|c|}
\hline
{\bf Parameter}	& {\bf Value}\\
\hline
File system size & 100 GB\\
\hline
Mean file size & 1 GB\\
\hline
No. of files & $\mathit{L} \cdot 100$\\
\hline
Disk block size & 4 KB\\
\hline
No. of block groups & 8\\
\hline
Disk blocks / bucket & 5120\\
\hline
Inode size & 281 bytes\\
\hline
IO Size & 32KB\\
\hline
\end{tabular}
\normalsize
%\vspace{-0.2cm}
%\caption[Experimental parameters]{Experimental parameters. L $\leftarrow$ File System Load factor.
%\label{hifs:table:expparameters}}
%\end{center}
%\end{table}
%


==> hifs/write.tex <==
\begin{algorithm}[H]
\caption{\emph{HIFS} write operation}
\label{hifs:algorithm:write}
\textbf{Procedure:} write\\
%\textbf{Desc:} perform file write operation at given offset.\\
\vspace{-0.5cm}
%----------------------------------------------------
\begin{algorithmic}[1]
\REQUIRE file path $f_{p}$, file offset $f_{o}$, data $\partial$, data length $\partial_{l}$\\
$\mathsf{I^{G_{n}}_{t}}$ : Inode tables, $\mathsf{B^{G_{n}}_{t}}$ : Disk Bucket Maps, $\mathsf{GD_{t}}$ : Group Descriptor table
\STATE \textless$i_{i}, i_{n}$\textgreater $\leftarrow$ SEARCH($\mathsf{I^{G_{n}}_{t}}$, $f_{p}$)
\STATE check file permissions in inode data
\STATE $b_{s} \leftarrow (\mathsf{d_{b_{n}}} * \mathsf{d_{s}})$, $w_{l} \leftarrow  0$
%\quad \quad \quad \COMMENT{disk bucket size in bytes}
%\STATE $f_{blk} \leftarrow (f_{o} / \mathsf{d_{s}})$		\quad \quad \quad \COMMENT{logical file block number}
%\STATE $f_{bkt} \leftarrow (f_{blk} / \mathsf{d_{b_{n}}})$	\quad \quad \COMMENT{logical file bucket number}
\WHILE{$w_{l} < \partial_{l}$}
	%\STATE $w_{l} \leftarrow  \partial_{l}$
	%\IF{$\partial_{l} > b_{s}$}
	%	\STATE $w_{l} \leftarrow b_{s}$
	%\ENDIF
	\STATE \textless$b_{i}, g_{i}$\textgreater $\leftarrow$ SEARCH($\mathsf{B^{G_{n}}_{t}}$, $\{f_{p}, f_{o}\}$)
	\IF{$b_{i}$ is null}
		\STATE \textless$b_{i}, g_{i}$\textgreater $\leftarrow$ INSERT($\mathsf{B^{G_{n}}_{t}}$, $\{f_{p}, f_{o}\}, \{\}$)
	\ENDIF
	%\STATE $f_{ob} \leftarrow f_{o} - (f_{bkt} * b_{s})$		\quad \COMMENT{write offset in bucket}
	\IF{$(\partial_{l} - w_{l}) > (b_{s} - (f_{o}$ mod $b_{s}))$}
		\STATE $\partial_{i} \leftarrow b_{s} - (f_{o}$ mod $b_{s})$
	\ELSE
		\STATE $\partial_{i} \leftarrow \partial_{l} - w_{l}$
	\ENDIF
	\STATE $s_{d} \leftarrow$ start offset of disk buckets in $\mathsf{GD}_{t}[g_{i}]$
	\STATE write $\partial[w_{l}:w_{l} + \partial_{i}]$ bytes to disk at offset $s_{d} + (b_{s} * b_{i}) + (f_{o}$ mod $b_{s})$
	\STATE $f_{o} \leftarrow f_{o} + \partial_{i}$,	$w_{l} \leftarrow w_{l} + \partial_{i}$
\ENDWHILE
\end{algorithmic}
\end{algorithm}


==> hinotationtable.tex <==
\begin{table}[t]
%
\vspace{0.2cm}
%\begin{center}
\tbl{Summary of notations\label{hitheory:table:notationtable}}{%
\begin{tabular}{|c|p{10cm}|}
\hline
{\bf Notation} & {\bf Description}\\
\hline
$s_{\phi}$ & Initial ADT state\\
\hline
$s^{\mathcal{M}}_{\phi}$ & Initial machine state\\
\hline
$s^{\mathcal{M}}_{0}$ & Initial data structure state\\
\hline
$s_{1}, s_{2}$ & ADT states\\
\hline
$s^{\mathcal{M}}_{1}, s^{\mathcal{M}}_{2}$ & Data structure (machine) states\\
\hline
$\delta$, $\delta_{1}$, $\delta_{2}$ & Sequences of ADT operations\\
\hline
$\delta^{\mathcal{M}}$, $\delta^{\mathcal{M}}_{1}$, $\delta^{\mathcal{M}}_{2}$ & Sequences of machine programs\\
\hline
$i, i_{1}, i_{2}$ & ADT inputs\\
\hline
$I, I_{1}, I_{2}$ & Sequences of ADT inputs\\
\hline
$\tau, \tau_{1}, \tau_{2}$ & ADT outputs\\
\hline
$i^{\mathcal{M}} = \alpha(i)$ & Denotes the machine representation of the ADT input $i$\\
\hline
$\tau^{\mathcal{M}} = \beta(\tau)$ & Denotes the machine representation of the ADT output $\tau$\\
\hline
$\gamma(o)$ & Denotes the machine program corresponding to the ADT operation $o$\\
\hline
$\delta^{\mathcal{M}} = \chi(\delta)$ & Denotes that $\delta^{\mathcal{M}}$ is a sequence of machine programs
corresponding to the ADT operation sequence $\delta$. If $\delta = \langle o_{1}, o_{2}, ..., o_{n} \rangle$ then
$\delta^{\mathcal{M}} = \langle \gamma(o_{1}), \gamma(o_{2}), ..., \gamma(o_{n}) \rangle$\\
\hline
$\mathbb{O}(\delta, s_{0}, I) \rightarrow (s_{n}, \tau_{n})$ & Denotes that the ADT operations sequence $\delta$ when applied to the ADT state $s_{0}$ with ADT input sequence $I$, results in the ADT state $s_{n}$ and ADT output $\tau_{n}$\\
\hline
$\mathbb{O}^{\mathcal{M}}(\delta^{\mathcal{M}}, s^{\mathcal{M}}_{0}, I) \rightarrow (s^{\mathcal{M}}_{n}, \tau^{\mathcal{M}}_{n})$ & Denotes that the program sequence $\delta^{\mathcal{M}}$ when applied to the machine state
$s^{\mathcal{M}}_{0}$ with ADT input sequence $I$, results in the machine state
$s^{\mathcal{M}}_{n}$ and machine output $\tau^{\mathcal{M}}_{n}$\\
\hline
\end{tabular}}
%\vspace{-0.2cm}
%\normalsize                      
%\caption{
%\label{hitheory:table:notationtable}}
%\vspace{-0.7cm}
%\end{center}
\end{table}

